Autonomy Loops for Monitoring, Operational Data Analytics, Feedback, and Response in HPC Operations

Many High Performance Computing (HPC) facilities have developed and deployed frameworks in support of continuous monitoring and operational data analytics (MODA) to help improve efficiency and throughput. Because of the complexity and scale of systems and workflows and the need for low-latency response to address dynamic circumstances, automated feedback and response have the potential to be more effective than current human-in-the-loop approaches which are laborious and error prone. Progress has been limited, however, by factors such as the lack of infrastructure and feedback hooks, and successful deployment is often site- and case-specific. In this position paper we report on the outcomes and plans from a recent Dagstuhl Seminar, seeking to carve a path for community progress in the development of autonomous feedback loops for MODA, based on the established formalism of similar (MAPE-K) loops in autonomous computing and self-adaptive systems. By defining and developing such loops for significant cases experienced across HPC sites, we seek to extract commonalities and develop conventions that will facilitate interoperability and interchangeability with system hardware, software, and applications across different sites, and will motivate vendors and others to provide telemetry interfaces and feedback hooks to enable community development and pervasive deployment of MODA autonomy loops.

==> Makefile <==
#
# Makefile
#

LATEXMK=latexmk -bibtex

MAIN=0position-paper-WAFVR-hpcmaspa

TEXFILES=$(wildcard *.tex)

all: $(TEXFILES)
	@$(LATEXMK) -pdf $(MAIN)
	@echo "Pending TODO items:"
	@grep TODO *.tex |grep -v newcommand | wc -l

force:
	@$(LATEXMK) -f -pdf $(MAIN)

clean:
	@$(LATEXMK) -c

distclean: clean
	@$(LATEXMK) -C

help:
	@echo -e "Usage : make [target]\n\
	all		produce the PDF (default)\n\
	force		force compilation if possilbe\n\
	clean		clean  unnecessary files\n\
	distclean	clean deeper\n\
	help		display this help"


